Excavating Vulnerabilities Lurking in Multi-Factor Authentication Protocols: A Systematic Security Analysis

Nowadays, cyberattacks are growing exponentially, causing havoc to Internet users. In particular, authentication attacks constitute the major attack vector where intruders impersonate legitimate users to maliciously access systems or resources. Traditional single-factor authentication (SFA) protocols are often bypassed by side-channel and other attack techniques, hence they are no longer sufficient to the current authentication requirements. To alleviate this problem, multi-factor authentication (MFA) protocols have been widely adopted recently, which helps to raise the security bar against imposters. Although MFA is generally considered more robust and secure than SFA, it may not always guarantee enhanced security and efficiency. This is because, critical security vulnerabilities and performance problems may still arise due to design or implementation flaws of the protocols. Such vulnerabilities are often left unnoticed until they are exploited by attackers. Therefore, the main objective of this work is identifying such vulnerabilities in existing MFA protocols by systematically analysing their designs and constructions. To this end, we first form a set of security evaluation criteria, encompassing both existing and newly introduced ones, which we believe are very critical for the security of MFA protocols. Then, we thoroughly review several MFA protocols across different domains. Subsequently, we revisit and thoroughly analyze the design and construction of the protocols to identify potential vulnerabilities. Consequently, we manage to identify critical vulnerabilities in ten of the MFA protocols investigated. We thoroughly discuss the identified vulnerabilities in each protocol and devise relevant mitigation strategies. We also consolidate the performance information of those protocols to show the runtime and storage cost when employing varying number of authentication factors.

==> 07_future_research_directions.tex <==
\section{Experimental results}\label{experimental_results}

==> 12_notes.tex <==
\section{Notes}

Notes during CSUV submission on 26 Jul 2024
    - Eliminated the HMACCE (protocol 1) paper table about AFs.
    - Eliminated Fig 5 of Protocol 2..

- We take a deep initiative to uncover the ceavates/xxx behind the design and implementation of exiting MFA protocols.

- Most of these protocols are published in top tier academic venues. 
    
## TODOs:
    - References for the orthogonal approaches
    - 

Outline:
    - Abstract
    - Introduction
    - Background
        - MFA
        - Auth Factors
    - Literature Review
        - MFA protocols across different domains
    - Threat Model
    - Security Analysis
        - Evaluation criteria
        - Security analysis
        - Performance Analysis
    - Suggested Mitigation Strategies
    - Conclusion 

Other notes:
- Removed Figure 4.
- Removed Figure 5.
- Table 3 can be removed.
- Figures moved to appendix: 6, ...

TODOs:
- Upper/lower cases for Gateway, Home, Device, ...
- ***PFS to be included. 
- Cite the most auth attacks...
- Estimated number of protocols reviewed?? 
- Cite AFs: knowledge, inherent, possession, ...
- Revise eval criteria
    - Include distinct AF (replace proper MFA) ...Done
    - Include AF independence ...Done
    - (Key) Leakage resilience: SK/key uncomputability from leaked sources and SK/key unpredictability (i.e., high entropy) ...Done
    - Include PFS ... Done 
    - Revise everything (Sec 5 \& 6) based on the revised criteria!!!!
- Define adversarial model
    - remove/change threat model
    - May use fig 4 and table 3.
    - Refer adversary assumption criteria to this model.
- Add future work in conclusion: formal analysis + expand scope in the PQ context


** New
    - Highlight the security requirements and constraints in different domains.
    - Complete the mitigation strategies.
    - Threat model???
    - List the AFs for the 10 MFA protocols discussed. 
    - Remove unnecessary figures in Appendix. 
    
    
    



